TESS Stellar Rotation up to 80 days in the Southern Continuous Viewing Zone

The TESS mission delivers time-series photometry for millions of stars across the sky, offering a probe into stellar astrophysics, including rotation, on a population scale. However, light curve systematics related to the satellite's 13.7-day orbit have prevented stellar rotation searches for periods longer than 13 days, putting the majority of stars beyond reach. Machine learning methods have the ability to identify systematics and recover robust signals, enabling us to recover rotation periods up to 35 days for GK dwarfs and 80 days for M dwarfs. We present a catalog of 7245 rotation periods for cool dwarfs in the Southern Continuous Viewing Zone, estimated using convolutional neural networks. We find evidence for structure in the period distribution consistent with prior Kepler and K2 results, including a gap in 10--20-day cool star periods thought to arise from a change in stellar spin-down or activity. Using a combination of spectroscopic and gyrochronologic constraints, we fit stellar evolution models to estimate masses and ages for stars with rotation periods. We find strong correlations between the detectability of rotation in TESS and the effective temperature, age, and metallicity of the stars. Finally, we investigate the relationships between rotation and newly obtained spot filling fractions estimated from APOGEE spectra. Field star spot filling fractions are elevated in the same temperature and period regime where open clusters' magnetic braking stalls, lending support to an internal shear mechanism that can produce both phenomena.

==> tables/cnn.tex <==
\begin{deluxetable*}{lcccccc}
\tablecaption{Convolutional Neural Network Architecture}
\tablehead{\colhead{Layer Type} & \colhead{Number of Filters} &\colhead{Filter Size} & \colhead{Stride} & \colhead{Activation} & \colhead{Dropout} & \colhead{Output Size}} 
\startdata
Input image &  -      & -             & -         & -         & -     & $64\times64$ \\
Conv2D      & $x$     & $3\times3$    & $1\times1$& ReLU      & -     & $62\times62\times x$\\
MaxPool2D   & 1       & $1\times3$    & $1\times3$& -         & 10\%  & $62\times20\times x$\\
Conv2D      & $y$     & $3\times3$    & $1\times1$& ReLU      & -     & $60\times18\times y$\\
MaxPool2D   & 1       & $1\times3$    & $1\times3$& -         & 10\%  & $60\times6\times y$\\
Conv2D      & $z$     & $3\times3$    & $1\times1$& ReLU      & -     & $58\times4\times z$\\
MaxPool2D   & 1       & $1\times4$    & $1\times4$& -         & 10\%  & $58\times1\times z$\\
Flatten     & -       & -             & -         & -         & -     & $58z$ \\
Dense       & -       & -             & -         & ReLU      & 10\%  & 256 \\
Dense       & -       & -             & -         & ReLU      & 10\%  & 64 \\
Dense       & -       & -             & -         & Softplus  & -     & 2 \\
\enddata
\label{tab:architecture}
\tablecomments{We used three 2D convolution layers with ReLU activation, max-pooling, and 10\% dropout. As in \citet{Claytor2022}, we used 2D max-pooling with a 1-dimensional kernel to pool in the time dimension, imparting translational invariance, but not the frequency dimension, to preserve frequency resolution. We tried four different combinations of filter numbers in the three convolution layers. We denote the number of filters as $x$, $y$, and $z$. The four runs had (A) $x=8$, $y=16$, and $z=32$ filters; (B) 16, 32, 64; (C) 32, 64, 128; (D) 64, 128, 256. The convolution output goes through a series of fully connected, or dense, layers, also with ReLU activation and 10\% dropout. Our architecture uses softplus output and negative log-Laplacian loss to predict the rotation period with its uncertainty.}
\end{deluxetable*}

==> tables/norot_table_columns.tex <==
\begin{deluxetable}{ll}
    \label{tab:norot}
    \centering
    %\tablewidth{\columnwidth}
    %\tabletypesize{\scriptsize}
    \tablecaption{Properties of \nnorot\ Rotationally Nondetected TESS SCVZ Stars}
    \tablehead{\colhead{Label} & \colhead{Description}}
    \startdata
        TIC     & TESS Input Catalog identifier \\
        TOI     & TESS Object of Interest identifier \\
        prov    & period provenance: TESS-SPOC or TASOC \\
        rvar    & photometric activity range $R_\mathrm{var}$ \\
        cdpp    & combined differential photometric precision \\
        Teff\_TIC   & TIC effective temperature \\
        Tmag    & TESS magnitude \\
        contratio   & TIC flux contamination ratio \\
        parallax    & \textit{Gaia} DR3 parallax \\
        ruwe    & \textit{Gaia} DR3 renormalized unit weight error \\
        phot\_g\_mean\_mag  & \textit{Gaia} DR3 apparent $G$ magnitude \\
        bp\_rp  & \textit{Gaia} DR3 $G_{BP} - G_{RP}$ color index \\
        teff    & APOGEE DR17 effective temperature \\
        teff\_err   & temperature uncertainty \\
        m\_h    & APOGEE DR17 metallicity [M/H] \\
        m\_h\_err   & metallicity uncertainty \\
        alpha\_m    & APOGEE DR17 $\alpha$ enhancement [$\alpha$/M] \\
        alpha\_m\_err   & $\alpha$ enhancement uncertainty \\
        star\_bad   & APOGEE DR17 stellar parameter fit flag \\
        snr\_bad    & APOGEE DR17 spectral signal-to-noise flag \\
    \enddata
    
    \tablecomments{The ``star\_bad'' flag represents the APOGEE stellar parameter fit flag, set when a best-fit model is close to a grid edge. It is set for 343 stars. The ``snr\_bad'' flag represents the APOGEE spectral signal-to-noise flag and is set for only 119 stars. This table is available in its entirety in machine-readable format.}
\end{deluxetable}


==> tables/rot_table_columns.tex <==
\begin{deluxetable}{ll}
    \label{tab:periods}
    \centering
    %\tablewidth{\columnwidth}
    %\tabletypesize{\scriptsize}
    \tablecaption{Properties of \nperiods\ Rotationally Detected TESS SCVZ Stars, MCMC Input \& Fit Parameters}
    \tablehead{\colhead{Label} & \colhead{Description}}
    \startdata
        TIC     & TESS Input Catalog identifier \\
        TOI     & TESS Object of Interest identifier \\
        prot    & CNN-inferred rotation period \\
        e\_prot & rotation period uncertainty \\
        prov    & period provenance: TESS-SPOC or TASOC \\
        spurious    & flag denoting likely spurious period \\
        rper    & photometric activity range $R_\mathrm{per}$ \\
        sph     & photometric activity index $S_\mathrm{ph}$ \\
        cdpp    & combined differential photometric precision \\
        Teff\_TIC   & TIC effective temperature \\
        Tmag    & TESS magnitude \\
        contratio   & TIC flux contamination ratio \\
        parallax    & \textit{Gaia} DR3 parallax \\
        ruwe    & \textit{Gaia} DR3 renormalized unit weight error \\
        phot\_g\_mean\_mag  & \textit{Gaia} DR3 apparent $G$ magnitude \\
        bp\_rp  & \textit{Gaia} DR3 $G_{BP} - G_{RP}$ color index \\
        teff    & APOGEE DR17 effective temperature \\
        teff\_err   & temperature uncertainty \\
        m\_h    & APOGEE DR17 metallicity [M/H] \\
        m\_h\_err   & metallicity uncertainty \\
        alpha\_m    & APOGEE DR17 $\alpha$ enhancement [$\alpha$/M] \\
        alpha\_m\_err   & $\alpha$ enhancement uncertainty \\
        snr\_bad    & APOGEE DR17 spectral signal-to-noise flag \\
        fspot   & spot filling fraction \\
        age     & MCMC gyrochronological age \\
        e\_age+  & 1$\sigma$ age upper credible limit \\
        e\_age-  & 1$\sigma$ age lower credible limit \\
        mass    & MCMC-inferred stellar mass \\
        e\_mass+ & 1$\sigma$ mass upper credible limit \\
        e\_mass- & 1$\sigma$ mass lower credible limit \\
        rad     & MCMC-inferred stellar radius \\
        e\_rad+  & 1$\sigma$ radius upper credible limit \\
        e\_rad-  & 1$\sigma$ radius lower credible limit \\
        Ro      & MCMC-inferred Rossby number \\
        fconv   & MCMC convergence flag \\
    \enddata
    
    \tablecomments{The ``snr\_bad'' flag represents the APOGEE spectral signal-to-noise flag and is set for only 21 stars. This table is available in its entirety in machine-readable format.}
\end{deluxetable}

